Polynomial Time Attack on Wild McEliece Over Quadratic Extensions

We present a polynomial time structural attack against the McEliece system based on Wild Goppa codes from a quadratic finite field extension. This attack uses the fact that such codes can be distinguished from random codes to compute some filtration, that is to say a family of nested subcodes which will reveal their secret algebraic description.

==> basics.tex <==


\section{McEliece Cryptosystem, Alternant and Goppa Codes}
\label{sec:basics}
\ac{Peut-\^etre le titre de cette section n'est-il plus si pertinent...}


\subsection{The McEliece scheme}
Recall here the general principle of McEliece's scheme. 
The key generation algorithm picks a random $k \times n$ generator matrix 
$\Gp$ of a code $\CC$ over $\Fqm$ 
which is itself randomly picked in a family of codes for
which $t$ errors can be corrected efficiently.
The \emph{secret} key is the decoding algorithm $\dec$ associated to $\CC$ and 
the \emph{public} key is $\Gp$. To encrypt $\uv \in \Fq^k$, the sender chooses
 a random vector $\ev$ in $\Fq^n$ of Hamming weight  $t$ and computes the ciphertext 
$\cv \eqdef \uv\Gp+\ev$. The receiver then recovers the plaintext by applying $\dec$ on $\cv$.


\smallskip

This describes the general scheme suggested by McEliece. From now on, we will say that $\Gp$ is the {\em public generator matrix} and that the vector space $\code{C}$ spanned by its rows is the {\em public code} \textit{i.e.}
$$
\code{C} \eqdef \{\uv \Gp ~|~ \uv \in \F_q^k\}.
$$
What is generally referred to as the McEliece cryptosystem is this scheme together with a particular choice of $\CC$, namely 
a binary Goppa code. This class of codes belongs to a more general class: the alternant code family  (\cite[Chap. 12, \S 2]{MacSloBook}).

\subsection{Alternant and Generalized Reed--Solomon codes}

\begin{definition}[Alternant code, support, degree, extension degree] 
The alternant code of degree $r$ over $\F_q$ associated to $\xv=(x_0,\dots,x_{n-1})\in (\fqm)^n$ (where all $x_i$'s are distinct) and $\yv=(y_0,\dots,y_{n-1})\in \left(\F^\times_{q^m}\right)^n$, denoted by
$\code{A}_r(\xv,\yv)$, is defined by
\begin{eqnarray}
\label{eq:description}
\code{A}_r(\xv,\yv)& \eqdef & \{\cv \in \F_{q}^n ~|~ \word{V}_{r}(\xv,\yv)  \cv^T={\bf 0}\},\\
\textrm{where}, \qquad \word{V}_{r}(\word{x},\word{y}) &\eqdef&
{\left(\begin{array}{lll}
y_0              & \cdots{} & y_{n-1}             \\
y_0 x_0           & \cdots{} & y_{n-1} x_{n-1}      \\
\vdots{}                &          & \vdots{}      \\
y_0 x_0^{r-1}    & \cdots{} & y_{n-1} x_{n-1}^{r-1}  
\end{array} \right)}.
\end{eqnarray}
The vector $\xv$ is called the {\em support} of $\code{A}_r(\xv,\yv)$, the integer $r$ is  its {\em degree} and
$m$ its {\em extension degree}.
\end{definition}

These codes are strongly related to Generalized Reed-Solomon (GRS) codes:
\begin{definition}[Generalized Reed-Solomon code] \label{def:defGRS}
Let $q$ be a prime power and
$k, n$ be integers such that $1 \leqslant k < n \leqslant q$.
Let $\xv$ and $\yv$ be two $n$-tuples such that the entries of $\xv$ are
pairwise distinct elements of $\fq$  and those of $\yv$ are nonzero elements in $\fq$.
% Alain suppression du "is".
% The Generalized Reed-Solomon code $\GRS{k}{\xv}{\yv}$ of dimension $k$ is associated to 
 The Generalized Reed-Solomon code $\GRS{k}{\xv}{\yv}$ of dimension $k$ associated to 
$(\xv,\yv)$ is the $k$-dimensional vector space $\GRS{k}{\xv}{\yv} \eqdef \left
\{(y_0p(x_0),\dots{},y_{n-1}p(x_{n-1})) \mid p \in \fq[z]_{< k} \right\}$.
Reed-Solomon codes correspond to the case
where $y_i=1$  for all $i \in \{0,\dots{},n-1\}$.
\end{definition}

A useful property of these codes is given in \cite[Chap. 12, \S 2]{MacSloBook}.
\begin{proposition}
  \label{prop:dualGRS} Let $\xv, \yv$ be as in 
  Definition \ref{def:defGRS}.
  Then,
  $$\GRS{k}{\xv}{\yv}^{\perp} = \GRS{n-k}{\xv}{\spc{\yv^{-1}}{\loc{\xv}'(\xv)^{-1}}},$$
where $\loc{\xv}$ is the locator polynomial of $\xv$ as defined in Section~\ref{subsec:poly}.
  \end{proposition}

This leads to this following alternative definition of alternant codes.
\begin{proposition}\label{pr:subfield_subcode}
The alternant code $\Alt{r}{\xv}{\yv}$ defined over $\fq$ where 
$\xv, \yv \in\fqm^n$ is the subfield subcode over $\Fq$ of the code
$\GRS{r}{\xv}{\yv}^{\perp}$
defined over $\fqm$, that is: %where
$$
\Alt{r}{\xv}{\yv} =  \GRS{r}{\xv}{\yv}^{\perp} \cap \fq^n.
$$
\end{proposition}

\begin{rem}
From Proposition~\ref{prop:dualGRS} and we deduce that
$$
\Alt{r}{\xv}{\yv} =  \GRS{n-r}{\xv}{\spc{\yv^{-1}}{\loc{\xv}'(\xv)^{-1}}} \cap \fq^n.
$$
\end{rem}
From this proposition it is clear that alternant codes inherit the decoding algorithms of 
the underlying GRS codes.
The key feature of an alternant code is the following fact (see \cite[Chap. 12, \S9]{MacSloBook}):
\begin{fact}
\label{fa:decoding}
There exists a polynomial time algorithm decoding all errors of Hamming weight at most $\lfloor \frac{r}{2} \rfloor$ once
a parity-check matrix $\Hm$ of the form $\Hm=\word{V}_{r}(\word{x},\word{y})$ is given for it.
\end{fact}

\subsection{Classical Goppa codes}
%Goppa codes form a subfamily of alternant codes.
% and are given by:
\begin{definition}[Classical Goppa codes, support and degree extension]\label{def:ClassicalGoppa}
Let $\xv=(x_0,\dots,x_{n-1})$ be an $n$--tuple of distinct elements 
of $\Fqm$, let $r$ be a positive integer and $\Gamma \in \Fqm[z]$
be a polynomial of degree $r$ such that $\Gamma (x_i)\neq 0$ for
all $i \in \{0, \ldots, n-1\}$.
The classical Goppa code $\Goppa{\xv}{\Gamma}$ over $\Fq$
associated to $\Gamma$ and supported by $\sv$
is defined as
$$
\Goppa{\xv}{\Gamma} \eqdef \Alt{r}{\xv}{\Gamma(\xv)^{-1}}.
$$
%alain : Je change tout.
% The  Goppa code $\code{G}(\xv,\pg)$ over $\F_q$ associated to a polynomial
% $\pg(z) \in \Fqm[z]$ of 
% degree $r$
% and an $n$-tuple $\xv=(x_0,\dots,x_{n-1})$ of distinct elements
% of $\fqm$ such that $\pg(x_i) \neq 0$ for all $i \in \{0,\dots{},n-1 \}$, is 
% the alternant code $\code{A}_r(\xv,\yv)$ of degree $r$
% with
% $y_i = \pg(x_i)^{-1}$.
We call $\Gamma$ the {\em Goppa polynomial},
$\xv$ the {\em support} and $m$
the {\em extension degree} of the Goppa code.
\end{definition}

The interesting point about this subfamily of alternant codes is that under some conditions, Goppa codes can correct more errors than a generic alternant code. 
\begin{proposition}[\cite{SKHN76}]
Let $\gamma(x)$ be a monic and square free polynomial. Let $\xv$ be an 
$n$-tuple $(x_0,\dots,x_{n-1})$ of distinct elements
of $\fqm$ satisfying $\gp(x_i) \neq 0$ for all $i$ in $\{0,\dots,n-1\}$.
% Alain, je fais un peu de cosmétique ici aussi.
Define
% alain : éduquons le lecteur
% $\yv=(y_i)_{0\leq i < n}$ by $y_i=\frac{1}{\gamma^{q-1}(x_i)}$ and 
% $\yv'=(y'_i)_{0\leq i < n}$ by $y'_i=\frac{1}{\gamma^{q}(x_i)}$.
% $$\yv \eqdef \left(\frac{1}{\gamma^{q-1}(x_0)}, \ldots ,
% \frac{1}{\gamma^{q-1}(x_{n-1})} \right) \quad \textrm{and} \quad 
% \yv' \eqdef \left(\frac{1}{\gamma^{q}(x_0)},\ldots ,
% \frac{1}{\gamma^{q}(x_{n-1})}  \right).$$
% Set $r=\deg \gp$, then
% $$
Set $r=\deg \gp$, then
% $$
% \code{A}_{(q-1)r}(\xv,\yv)=\code{G}(\xv,\gamma^{q-1}(x))=\code{G}(\xv,\gamma^{q}(x))=\code{A}_{qr}(\xv,\yv').
% $$
$$
\code{A}_{(q-1)r}(\xv,\gamma^{-(q-1)}(\xv))=\code{G}(\xv,\gamma^{q-1})=\code{G}(\xv,\gamma^{q})=\code{A}_{qr}(\xv,\gamma^{-q}(\xv)).
$$
\end{proposition}

From Fact \ref{fa:decoding}, these Goppa codes correct up to
$\lfloor \frac{qr}{2}\rfloor$ errors in polynomial-time instead
of just $\lfloor \frac{(q-1)r}{2}\rfloor$ if viewed as
%alain
as
%$\code{A}_{(q-1)r}(\xv,\yv)$.
$\code{A}_{(q-1)r}(\xv,\gamma^{-(q-1)}(\xv))$.
Notice that when $q=2$, this amounts to double the error correction capacity.
It is one of the reasons why binary Goppa codes have been chosen in the original McEliece scheme or why Goppa codes with Goppa polynomials of the form $\gp^ {q-1}$ (called {\em wild Goppa codes}) are proposed in \cite{BLP10a, BLP11a}.

\subsection{Wild Goppa codes over quadratic extensions}
When the extension degree $m$ equals $2$, wild Goppa codes have additional
properties which are summarized in Proposition ~\ref{pr:properties_superGoppa}
below. 

\begin{proposition}[{\cite{COT13}}]\label{pr:properties_superGoppa}
Let $\Goppa{\xv}{\gamma^{q-1}(z)}$ be a wild Goppa code of length $n$, defined over $\fq$ 
with support $\xv \in \Fqq^n$ where  $\gamma(z) \in \Fqq[z]$ is assumed to be irreducible of degree $r>1$. Then
\begin{enumerate}[(i)]
\item\label{it:superGoppa} $\Goppa{\xv}{\gamma^{q-1}(z)}  =  \Goppa{\xv}{\gamma^{q+1}(z)} $;
\item\label{it:rrmoins2} $\dim(\Goppa{\xv}{\gp^{q+1}(z)})  \geq  n - 2r(q-1) + r(r-2)$;
\item\label{it:PsupSRS} There exists $\yv \in \Fq^n$
such that $\Goppa{\xv}{ \gp^{q+1}} = \sP{\yv}{\Alt{r(q+1)}{\xv}{\loc{\xv}'(\xv)^{-1}}}$.
\end{enumerate}
\end{proposition}

\begin{proof}
The results (\ref{it:superGoppa}), (\ref{it:rrmoins2})
and (\ref{it:PsupSRS}) are respective straighforward consequences of
Theorem 1, Theorem 24 and Corollary 10 of \cite{COT13}.
\end{proof}

\begin{rem}
  About Proposition~\ref{pr:properties_superGoppa}~(\ref{it:PsupSRS}),
notice that the code $\Alt{r(q+1)}{\xv}{\loc{\xv}'(\xv)^{-1}}$ is nothing but
the subfield subcode of a shortened Reed--Solomon code, that is a shortened
BCH code.
\ac{Ouais, sous cette forme c'est peut-\^etre un peu sec, par contre \c{c}a permet de virer la notation SRS. Il faudra peut-\^etre d\'etailler un chouilla.}
\end{rem}

\subsection{Duality, shortening, puncturing, subfield subcodes and trace codes}
The following classical results will be used repeatedly.

 \begin{lem}
 \label{lem:dualshort}
 Let $\code{A} \subset \Fqm^n$ be a code and $\Ind \subset \{0, \ldots , n-1\}$
   be a set of positions.  Then,
   $$
   {(\sh{\code{A}}{\Ind})}^{\perp} = \pu{\left(\code{A}^{\perp}\right)}{\Ind}
   \quad \textrm{and}\quad
   {(\pu{\code{A}}{\Ind})}^{\perp} = \sh{\left(\code{A}^{\perp}\right)}{\Ind}.
   $$
 \end{lem}
 
\ac{Preuve????}

 \jp{J'aime pas ma référence plus bas, ce serait mieux d'avoir une référence de l'endroit où a été publié
 le résultat de Delsarte + référence accessible complémentaire éventuellement. Vu ma connexion internet, je préfère
 faire cela plus tard, à moins qu'Ayoub le fasse.}
 \begin{theorem}[Delsarte's Theorem, { see \cite[Thm 7.11]{MacSloBook}}]
 \label{th:Delsarte}
 Let $\code{E}$ be a linear code of length $n$ defined over $\Fqm$.
 Then 
 $$
 (\code{E} \cap \Fq^n)^\perp = \tr(\code{E}^\perp).
 $$
 where $\tr$ stands for the component wise trace map from $\Fqm$ to
 $\Fq$.
 \end{theorem}

The following elementary statement is extremely useful in the next sections.

\begin{proposition}\label{prop:commutation}
  Let $\code{A}$ be a code over $\Fqm$ of length $n$ and $\Ind \subset
  \{0, \ldots , n-1\}$, then, we have
  $$
  \begin{aligned}
    \sh{\code{A}}{\Ind} \cap \Fq^{n - |\Ind|} & =
        \sh{(\code{A} \cap \Fq^n)}{\Ind} \qquad \qquad
    &\pu{\tr(\code{A})}{\Ind} & =
        \tr (\pu{\code{A}}{\Ind})\\
        \pu{(\code{A}\cap \Fq^n)}{\Ind} &\subseteq \pu{\code{A}}{\Ind}
        \cap \Fq^{n-|\Ind|} \qquad \qquad
        &\tr(\sh{\code{A}}{\Ind}) &\subseteq \sh{\tr (\code{A})}{\Ind}.
  \end{aligned}
  $$
  and the converse inclusions are false in general.
\end{proposition}

\begin{proof}
  It is an elementary exercise of linear algebra.
\end{proof}

\subsection{Shortening alternant codes}
\begin{proposition}\label{pr:shortened_alternant_code}
Let $\xv$ be an $n$--tuple of pairwise distinct elements in $\fqm$,
$\yv$ be an $n$--tuple of nonzero elements of $\fqm$ and $\pg \in \fqm[z]$, 
then,
\begin{eqnarray}
\label{eq:shortAlt}\sh{\Alt{r}{\xv}{\yv}}{\Ind} & = &
\Alt{r}{\xv_{\Ind}}{\yv_{\Ind}}\\
\label{eq:shortGop}\sh{\Goppa{\xv}{\pg}}{\Ind} & = & \Goppa{\xv_{\Ind}}{\pg}.
\end{eqnarray}
\end{proposition}

\begin{proof}
From Lemma~\ref{lem:dualshort}, we have
\begin{equation}\label{eq:dualternant}
{\left(\sh{\Alt{r}{\xv}{\yv}}{\Ind}\right)}^{\bot} = 
\pu{(\Alt{r}{\xv}{\yv}^{\bot})}{\Ind}
\end{equation}
Moreover, from Proposition~\ref{pr:subfield_subcode} together with
Theorem~\ref{th:Delsarte}, we have
$$
(\Alt{r}{\xv}{\yv}^{\bot}) = \tr (\GRS{r}{\xv}{\yv}). 
$$
From Proposition~\ref{prop:commutation}, we get
\begin{eqnarray}
\pu{(\Alt{r}{\xv}{\yv}^{\bot})}{\Ind} &=& \pu{\tr (\GRS{r}{\xv}{\yv})}{\Ind} \\
 &=& \tr \left( \pu{\GRS{r}{\xv}{\yv}}{\Ind}\right)\\
\label{eq:trGRS} &=& \tr  \left( \GRS{r}{\xv_{\Ind}}{\yv_{\Ind}}\right)
\end{eqnarray}
Putting~(\ref{eq:dualternant}) together with (\ref{eq:trGRS})
and applying Theorem~\ref{th:Delsarte} again, we get 
$$
\begin{aligned}
\sh{\Alt{r}{\xv}{\yv}}{\Ind} &= {\left(\tr (\GRS{r}{\xv_{\Ind}}{\yv_{\Ind}}) \right)}^{\bot}\\
 &= \GRS{r}{\xv_{\Ind}}{\yv_{\Ind}}^{\bot} \cap \Fq^{n-|\Ind|}\\
 & = \Alt{r}{\xv_{\Ind}}{\yv_{\Ind}}.  
\end{aligned}
$$
This proves~(\ref{eq:shortAlt}). Then, (\ref{eq:shortGop}) is obtained from
(\ref{eq:shortAlt}) and Definition \ref{def:ClassicalGoppa}.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "article"
%%% End: 


==> context.tex <==
\section{The main tool of the attack : a filtration which reveals the algebraic structure}\label{sec:Context}



% %.
%

%
%
%\begin{rem}
%As said above, the polynomial $\gamma$ is assumed to be irreducible.
%Actually, one can prove that
%the presently described attack still works if $\gamma$
%is squarefree with no roots in $\Fqq$. Indeed, this relaxed
%hypothesis is sufficient to apply the results of \cite{COT13}
%which are necessary to perform the attack.
%\end{rem}

\ao{Pas s\^ur que tout ce qui suit devrait rester..\\
Finally, in order to recover the secret support vector $\xv$, we will need
the following lemma fundamental to the attack.
\begin{lemma}
  \label{lem:starNorm}
  Let $\code{A}$ be a code over $\Fqq$ and $\cv\in \Fq^n$, then
  \begin{equation}\label{eq:starFq}
  \spc{\cv}{(\code{A}\cap \Fq^n)} = (\spc{\cv}{\code{A}})\cap \Fq^n\quad
  \textrm{and}\quad \spc{\cv}{\tr(\code{A})} = \tr(\spc{\cv}{\code{A}}).
  \end{equation}
  In particular, for all $\zv\in \Fqq^n$, we have
  \begin{equation}\label{eq:starNorm}
  \spc{\zv^{q+1}}{(\code{A}\cap \Fq^n)} = (\spc{\zv^{q+1}}{\code{A}})\cap \Fq^n
  \quad \textrm{and}\quad \spc{\zv^{q+1}}{\tr(\code{A})} = 
  \tr(\spc{\zv^{q+1}}{\code{A}}).
  \end{equation}
\end{lemma}
\begin{proof}
  The proof of (\ref{eq:starFq}) is elementary.
  To prove (\ref{eq:starNorm}), notice that $\zv^{q+1}$ is nothing but
  its norm $\nr (\zv)$ and hence is an element of $\Fq^n$. 
  Thus (\ref{eq:starNorm}) is a consequence of (\ref{eq:starFq}).
\end{proof}
\begin{corollary}
  \label{cor:AstarBFq}
  Let $\code{A}, \code{B}$ be two codes of length $n$ over $\Fqq$, then
  $$
  \spc{(\code{A}\cap \Fq^n)}{\tr(\code{B})} \subseteq \tr(\spc{\code{A}}{\code{B}}).
  $$
\end{corollary}}
\ac{Le probl\`eme c'est qu'on en a besoin pour prop~\ref{prop:doubleinj}}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "article"
%%% End: 


==> pseudocode.tex <==
\section{Pseudo-code of the attack}

\begin{algorithm}
 \caption{\label{al:total} Algorithm of the attack.}
\begin{algorithmic}
\STATE{Compute $\Coi{0}{q+1}$, $\Coi{1}{q+1}$ using 
Algorithm \ref{al:sCoi0v}.}
\STATE{$ L_0 \leftarrow$ List of candidates for $\xvzero^{q+1}$ (Obtained by solving System ($S_0$) in (\ref{eq:norms}))}
\STATE{$ L_1 \leftarrow$ List of candidates for $(\xvone-1)^{q+1}$
 (Obtained by solving System ($S_1$) in (\ref{eq:norms}))}
\STATE{$\mat{M}_0 \leftarrow 0$}
\WHILE{$\mat{M}_0=0$ and $L_0 \neq \emptyset$}
\STATE{Pick a random element $\av_0$ in $L_0$.}
\STATE{$\av_1 \leftarrow \phi(\av_0)$}
\STATE{$L_0 \leftarrow L_0 \setminus \{\av_0\}$}
\COMMENT{where $\phi$ is the map of Lemma~\ref{lem:pairs}.}
\STATE{$L_1 \leftarrow L_1 \setminus \{\av_1\}$}
\STATE{ Compute the minimal polynomials $P_i$ of the positions using Section
\ref{ss:Step4}.}
\STATE{Construct a permuted generator matrix  $\Gsige$ of $\CCse$ (the code $\CCs$ extended by zero see Section \ref{ss:ESpp}) and
a parity-check matrix $\mat{H}$ of the target code $\TC$ 
as described in Section~\ref{ss:Step4}.}
\STATE{$V \leftarrow$ Space of solutions $\mat{M}$ of
$\mat{H}\left( \Gsige \mat{M} \right)^T=0$}
\IF{$\dim V>0$ and $\exists \mat{M} \in V$ satisfying conditions (\mat{M}1)
and (\mat{M}2) (see Section~\ref{ss:Step4})}
\STATE{$\mat{M}_0 \leftarrow M$}
\ENDIF
\ENDWHILE
\IF{$\mat{M}_0=0$}
\RETURN{``error''}
\ELSE
\STATE{Recover $\xv$ and $\yv$ from $\mat{M}$ (See Section \ref{ss:finalStep}).}
\RETURN{$\xv, \yv$}
\ENDIF
\end{algorithmic}
\end{algorithm}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "article"
%%% End: 

